On abstract normalisation beyond neededness

We study normalisation of multistep strategies, strategies that reduce a set of redexes at a time, focussing on the notion of necessary sets, those which contain at least one redex that cannot be avoided in order to reach a normal form. This is particularly appealing in the setting of non-sequential rewrite systems, in which terms that are not in normal form may not have any needed redex. We first prove a normalisation theorem for abstract rewrite systems (ARS), a general rewriting framework encompassing many rewriting systems developed by P-A.Melli\`es in his PhD thesis. The theorem states that multistep strategies reducing so called necessary and never-gripping sets of redexes at a time are normalising in any ARS. Gripping refers to an abstract property reflecting the behavior of higher-order substitution. We then apply this result to the particular case of PPC, a calculus of patterns and to the lambda-calculus with parallel-or.

==> dibujo.tex <==
\begin{wrapfigure}[3]{l}{0.2\textwidth}
\vspace{-1mm}
\minicenter{
\newcommand{\testigo}{}
\newcommand{\alturasub}{-0.1}
\newcommand{\alturanorm}{0}
\newcommand{\anchomult}{0.85}
\newcommand{\lebend}{90}
\begin{tikzpicture}%[remember picture,overlay,baseline=(primerlambda.base)]
  \node (formula) {$\lp{\set{x}} \ x \ \wid{x} \ . \ x \ \wid{x}$};
  \node (subxuno) at (-0.73 * \anchomult,\alturasub) {\testigo};
  \node (subxdos) at (-0.7 * \anchomult,\alturasub) {\testigo};
  \node (matx) at (0.17 * \anchomult,\alturanorm) {\testigo};
  \node (varx) at (0.7 * \anchomult,\alturanorm) {\testigo};
  \draw[->, thick] (subxuno) to[bend right=80] (matx);
  \draw[->, thick] (subxdos) to[bend right=\lebend] (varx);
\end{tikzpicture}
}
%\caption{Free/bound variables/matchables}\label{fig:free-bound}
\end{wrapfigure}

